Meta-Evolve: Continuous Robot Evolution for One-to-many Policy Transfer

We investigate the problem of transferring an expert policy from a source robot to multiple different robots. To solve this problem, we propose a method named $Meta$-$Evolve$ that uses continuous robot evolution to efficiently transfer the policy to each target robot through a set of tree-structured evolutionary robot sequences. The robot evolution tree allows the robot evolution paths to be shared, so our approach can significantly outperform naive one-to-one policy transfer. We present a heuristic approach to determine an optimized robot evolution tree. Experiments have shown that our method is able to improve the efficiency of one-to-three transfer of manipulation policy by up to 3.2$\times$ and one-to-six transfer of agile locomotion policy by 2.4$\times$ in terms of simulation cost over the baseline of launching multiple independent one-to-one policy transfers.

==> section_exp_design.tex <==



\section{Experimental Design}

For fair comparison of different approaches, the hyperparameters that ensure optimal performance should be searched for each method. 
In this section, we present the process we used to search the (near-)optimal hyperparameters for both our Meta-Evole and HERD to allow easy re-production of our experiment results.
We found that Meta-Evolve and HERD share the same set of hyperparameters while achieving their own optimal performance.

\textbf{Basic RL Hyperparameters. }
In HERD and our Meta-Evolve experiments, we followed the same settings for the basic RL hyperparameters as in the DAPG \cite{dapg}.
This allows us to also fairly compare against DAPG \cite{dapg} in our experiments.
These basic RL hyperparameters include discount factor $\gamma$, GAE, NPG step size, policy and value network sizes, epoch length, and batch size.


\textbf{Evolution Progression Step Size $\xi$. }
We start the searching of $\xi$ from a small value and increase it until the evolution becomes too aggressive and the policy transfer start to fail.
Specifically, we searched among $\{0.001, 0.005, 0.01, 0.02, 0.03, 0.06, 0.1 \}$ and noticed that the policy transfer starts to fail at $0.1$.
Therefore, we adopted $0.06$ for the best policy transfer efficiency.

\textbf{Number of Sampled Evolution Parameter Vectors for Jacobian Estimation. }
To estimate the Jacobian, the number of sampled evolution parameter vectors should be larger than the dimension of evolution parameters $D$.
At the same time, it should be as small as possible for better simulation efficiency.
For HMS tasks, we searched among $\{72, 84, 96, 120\}$ and found that $72$ is enough to ensure good estimation of Jacobian and yield overall best efficiency among other searched numbers.
For locomotion tasks, we searched among $\{12, 24, 36\}$ and found $12$ achieves the best overall efficiency.

\textbf{Evolution Direction Weighting Factor $\lambda$. }
Evolution direction weighting factor $\lambda$ determines the impact of the reward on the evolution direction.
A smaller $\lambda$ would allow the reward to play a larger role of deciding the evolution direction.
At the same time, it should be larger than or equal to $1$ to ensure that evolution parameter $\alpha$ converge to the target robots.
We searched among $\{1, 1.05, 1.1, 1.2\}$ and found that using $\lambda=1$ yield the best overall efficiency in policy transfer.

\textbf{Sample Range Shrink Ratio. }
We start searching shrink ratio of intermediate robot sample range from 1 (which means no shrinking) and then decrease it improve adaptation toward the next intermediate robot.
Specifically, we searched among $\{1, 0.995, 0.99, 0.98\}$ and found that $0.995$ can ensure successful policy transfer while also achieves the best efficiency.

\textbf{Success Rate Threshold for Moving to the Next Training Phase. }
We used success rate as the indicator for deciding whether to move on to the next intermediate robot during policy transfer.
Specifically, the policy transfer moves on to the next intermediate robot if and only if the success rate on the current intermediate robot exceeded a certain threshold.
We searched success rate threshold among $\{0.4, 0.5, 0.6, 0.667, 0.7, 0.75, 0.8\}$ and found that $0.667$ achieves the best efficiency.

